Causally Debiased Latent Action Model for Embodied Action-Conditioned World Models

Action-conditioned world models (ACWMs) aim to simulate future observations conditioned on embodied actions. However, learning controllable ACWMs requires large-scale action-labeled data, which remains costly to collect. Latent action models (LAMs) mitigate this bottleneck by inferring latent actions from videos without executable action labels, but existing LAMs are typically trained with reconstruction-only objectives and therefore entangle action-relevant dynamics with action-irrelevant visual confounders. With such objectives, LAM favors visual context over action dynamics, therefore downstream ACWMs exhibit residual motion under zero actions and fail to reproduce supplied dynamics. We propose CD-LAM, a causally debiased framework for LAM-based ACWMs. CD-LAM introduces three debiasing objectives: embodiment-centric reconstruction, action-centric contrastive learning, and latent space calibration, which together encourage embodiment-focused, action-aware, and well-calibrated representations. CD-LAM reduces action-following error by up to 42% and 35% when conditioned on latent and robot actions, while improving fidelity, and matching DreamDojo reference with over 12$\times$ fewer adaptation updates. CD-LAM also adapts LTX-2.3-22B into an ACWM with competitive quality using only 3.2% of DreamDojo-14B's sample exposures. On X-VLA, pretraining with CD-LAM instead of baseline LAM consistently improves success rates by up to 5 percent point across LIBERO, LIBERO-Plus, and RoboTwin C2R.

==> 00_abstract.tex <==
\abstract{

Action-conditioned world models (ACWMs) aim to simulate future observations conditioned on embodied actions. 
However, learning controllable ACWMs requires large-scale action-labeled data, which remains costly to collect. Latent action models (LAMs) mitigate this bottleneck by inferring latent actions from videos without executable action labels, but existing LAMs are typically trained with reconstruction-only objectives and therefore entangle action-relevant dynamics with action-irrelevant visual confounders. 
With such objectives, LAM favors visual context over action dynamics, therefore downstream ACWMs exhibit residual motion under zero actions and fail to reproduce supplied dynamics.
We propose CD-LAM, a causally debiased framework for LAM-based ACWMs. CD-LAM introduces three debiasing objectives: embodiment-centric reconstruction, action-centric contrastive learning, and latent space calibration, which together encourage embodiment-focused, action-aware, and well-calibrated representations. CD-LAM reduces action-following error by up to 42\% and 35\% when conditioned on latent and robot actions, while improving fidelity, and matching DreamDojo reference with over 12$\times$ fewer adaptation updates. CD-LAM also adapts LTX-2.3-22B into an ACWM with competitive quality using only 3.2\% of DreamDojo-14B's sample exposures. On X-VLA, pretraining with CD-LAM instead of baseline LAM consistently improves success rates by up to 5\% across LIBERO, LIBERO-Plus, and RoboTwin C2R.




}


==> 01_introduction.tex <==
\section{Introduction}

Action-conditioned world models (ACWMs)~\citep{ha2018worldmodels,hafner2023dreamerv3,acwmphys2026,wu2024ivideogpt} have emerged as a promising paradigm for simulating the physical world directly from visual observations and embodied control signals. Given the current observation and an action trajectory, an ACWM aims to forecast the resulting future observation sequence, thereby simulating how the environment and embodiment would evolve under that intervention. By predicting futures under different candidate action trajectories, ACWMs have the potential to serve as general-purpose simulators for robot planning, policy evaluation, and data augmentation.
%oxe2023
However, the controllability of ACWMs relies on large-scale action-labeled data, yet collecting robot videos with action annotations remains costly in the real world~\citep{khazatsky2024droid}. In contrast, human videos are easier to collect, far more scalable, and rich in physical interactions, but they typically lack executable action annotations~\citep{grauman2022ego4d,grauman2024egoexo4d,damen2018epic}. Latent action models (LAMs) offer a bridge to such large-scale data sources by inferring compact latent action representations from unlabeled video transitions~\citep{bruce2024genie,schmidt2024lapo,ye2024lapa}. Through large-scale pre-training conditioned on these latent actions, ACWMs can be effectively warmed up to learn action-controllable dynamics and achieve stronger action-following performance after fine-tuning on limited labeled robot data~\citep{gao2025adaworld,dreamdojo2026}.

Despite this promise, existing LAMs are typically trained solely with the video reconstruction objective, which cannot prevent action-irrelevant visual factors from being encoded into the latent actions. In particular, action-irrelevant factors such as background scenes and non-interacted objects may leak into the latent action representation. Our analysis in Section~\ref{sec:confounder} shows that such action-irrelevant factors induce biased latent action representations, which ultimately confound the ACWM: the model can generate visually plausible rollouts, but fails to reliably follow the supplied actions ~\citep{zhang2025whatdolams,nikulin2025latentdistractors,conla2026}. The inclusion of these confounders in the action condition can leave the ACWM with a biased state for robot-action adaptation and impose an additional alignment burden. We introduce latent-space diagnostics and intervention-based evaluations to visualize and quantify such bias. Our diagnostic results reveal substantial responses to small camera shifts and shortcuts that favor visual context over action similarity. Evaluation results further expose weak action following under both latent-action and robot-action conditioning, including residual motion under zero-action inputs and failure to reproduce target dynamics.

% Our diagnostics reveal that action-irrelevant confounders distort latent-action representations, allowing visual context to outweigh action signal, while interventions expose action-following failures that persist from latent-action conditioning to robot-action conditioning.  Together, these findings identify an upstream problem: the latent action condition itself is already confounded before robot-action adaptation, leaving executable controls to be aligned with a partly non-actionable latent space.

% Concretely, we introduce three causally debiased objectives for LAMs: embodiment-centric reconstruction, action-centric contrastive learning, and latent space calibration, which respectively encourage embodiment-focused, action-aware, and calibrated action representations. The debiasing stages require no executable action labels and the contrastive objective uses only coarse task or verb annotations when available.

\begin{figure}[!t]
\centering
\includegraphics[width=1 \linewidth]{figures/fig1_iclr.pdf}
\caption{\textbf{Performance overview and confounding analysis.}
CD-LAM lowers action-following error (FDCE) and raises PSNR at both 2B and 14B scales, with much lower training cost than DreamDojo. A reconstruction-trained LAM can leak action-irrelevant confounders into the action condition, and CD-LAM reduces this shortcut dependence.}
\label{fig:overall}\label{fig:causal}
\end{figure}%
Motivated by these findings, we propose CD-LAM to address action-irrelevant confounding in LAM-based ACWMs by explicitly shaping the latent action space. Specifically, it combines embodiment-centric reconstruction to emphasize the embodiment and interacted objects over background, action-centric contrastive learning to group transitions by coarse primitives across visual confounders and mitigate visual-context-driven shortcuts, and latent space calibration to suppress spurious responses to unchanged observations. CD-LAM consists of an efficient three-stage fine-tuning pipeline (Figure~\ref{fig:arch}) that first debiases the LAM, then the ACWM, and finally adapts the ACWM to real-world robot actions. In Stage 1, we fine-tune the LAM with these three debias objectives to emphasize embodiment-centric action dynamics. In Stage 2, we fine-tune the ACWM on debiased latent actions extracted from human videos without executable action labels, to debias the learned controllability and improve action following under the corrected latent conditions. In Stage 3, we add a lightweight action-to-latent-action mapping layer to bridge robot actions into the debiased latent space as the conditioning input and adapt the ACWM to executable robot controls. 

% The first two stages require no executable action labels and the contrastive objective uses only coarse task or verb annotations when available.

% Beyond this, we further explore the usage of the latent-action interface on the 22B LTX-2.3 video backbone and X-VLA policy pretraining~\citep{hacohen2026ltx2,zheng2025xvla}.

Experiments on 2B and 14B backbones show that upstream latent-action debiasing improves downstream world-model controllability (Figure~\ref{fig:overall}; Section~\ref{sec:experiments}). Before robot-action alignment, CD-LAM reduces action-following error, measured by Foreground Displacement Chamfer Error (FDCE), by 42\% and 26\%, respectively. These gains persist after \ratstage{}, with FDCE reductions of 35\% and 30\% alongside improved visual fidelity. The complete pipeline also matches the released DreamDojo reference with more than 12\(\times\) fewer \ratstage{} updates. Beyond DreamDojo, CD-LAM enables efficient adaptation of the pretrained 22B LTX-2.3 video backbone~\citep{lightricks2026ltx23} into an ACWM conditioned on executable robot actions. The resulting model achieves comparable rollout quality while using 3.2\% of the sample exposures reported for DreamDojo-14B across latent-action finetuning and robot-action adaptation. For policy learning, pretraining X-VLA~\citep{zheng2025xvla} with CD-LAM rather than the original LAM improves success rates across LIBERO, LIBERO-Plus and RoboTwin C2R~\citep{liu2023libero, fei2025liberoplus,chen2025robotwin}. 

This paper makes three contributions: 

% \begin{itemize}
$\bullet$ We identify and analyze a confounding mechanism in LAM-based ACWMs: action-irrelevant visual factors enter the latent action condition and undermine downstream controllability. %We introduce latent-space diagnostics and intervention-based evaluations to characterize this failure.

$\bullet$ We propose CD-LAM, a causally motivated framework that targets this bias at its source by learning debiased action representations for world-model fine-tuning and executable robot-action alignment.

$\bullet$ %We demonstrate that upstream representation correction
Our CD-LAM yields persistent improvements on action-conditioned world models DreamDojo-2B/14B and LTX-2.3-22B, also improving policy models in three robot manipulation benchmarks.
%: controllability gains survive robot-action adaptation, while the resulting framework supports efficient world-model adaptation and more robust policy learning.
% We have released the debiased LAMs and ACWMs checkpoints, evaluation protocols, and training code at \url{https://anonymous.4open.science/r/CD-LAM-anonymous-373C/}..



==> 02_preliminaries.tex <==
\section{Preliminaries}
\label{sec:prelim}

\noindent\textbf{Action-conditioned world models.}\label{sec:prelim-acwm} An action-conditioned world model~(ACWM) predicts future observations under an action sequence:
 \begin{equation}
    p_\theta(o_{t+1:t+H}\mid o_{\leq t}, u_{t:t+H-1}),
    \label{eq:acwm-real-action}
\end{equation}
where \(o_t\) denotes the visual observation at time \(t\) and \(u_t\) denotes a recorded executable robot action, such as a relative end-effector displacement.

\noindent\textbf{Latent action models.}\label{sec:prelim-lam}
Given adjacent frames $\langle o_t,o_{t+1} \rangle$, the LAM infers a latent action vector \(z_t \in \mathbb{R}^d\), \ie a summary of the observed action-related information~\citep{bruce2024genie,schmidt2024lapo,ye2024lapa}.
A LAM can be written as an encoder paired with a decoder:
\begin{equation}
    z_t \sim q_\phi(z\mid o_t,o_{t+1}),
    \qquad
    \hat{o}_{t+1}=D_\psi(o_t,z_t).
    \label{eq:lam-autoencoder}
\end{equation}
We write \(\mu_\phi(o_t,o_{t+1})\) for the posterior mean of \(q_\phi\), used whenever a deterministic latent action is needed.
The standard LAM objective is next-frame reconstruction, optionally with a bottleneck or prior regularizer:
\begin{equation}
    \mathcal{L}_{\mathrm{LAM}}
    =
    \mathbb{E}\big[
        \ell(D_\psi(o_t,z_t),o_{t+1})
    \big]
    +
    \mathrm{Reg}(z_t).
    \label{eq:lam-loss}
\end{equation}
Here \(\ell\) is the observation reconstruction loss, and \(\mathrm{Reg}\) denotes the capacity-control mechanism used by the particular LAM, such as a KL bottleneck. This objective defines $z_t$ by information that helps reconstruct or predict the observed transition.

\noindent\textbf{Latent action conditioning.}\label{sec:prelim-latent-acwm} Prior LAM-based ACWM systems use latent actions as substitutes for missing robot actions during ACWM training on egocentric video: transitions are encoded as \((o_t,o_{t+1}) \mapsto z_t\), and the world model is trained as
\begin{equation}
    p_\theta(o_{t+1:t+H}\mid o_{\leq t}, z_{t:t+H-1}).
    \label{eq:latent-acwm}
\end{equation}
This pipeline requires two properties. The latent action should capture the embodied action in the observed transition, and the world model should make future motion follow the latent action condition~\citep{gao2025adaworld,dreamdojo2026}.  
Note that \(z_t\) plays a different role from \(u_t\): a recorded robot action \(u_t\) is an executable control signal defined by an embodiment and its controller, whereas \(z_t\) is a video-derived conditioning variable defined solely by the LAM training objective.


==> 02_related_work.tex <==
\section{Related Work}\label{sec:related}
\indent{\textbf{\textit{Latent Action Learning from Video.}}}
Latent action learning builds on observation-only imitation~\citep{edwards2019ilpo} and video-based pretraining with inferred action labels~\citep{baker2022vpt}. Genie~\citep{bruce2024genie} learns discrete latent controls for interactive generation, while LAPO~\citep{schmidt2024lapo} uses inferred actions to bootstrap policies and shows that improved reconstruction need not yield better policy learning. LAPA~\citep{ye2024lapa} and Moto~\citep{chen2024moto} use quantized transition representations for policy pretraining: LAPA replaces its latent prediction head during robot-action fine-tuning, whereas Moto retains motion-token supervision. These works establish the value of video-derived action targets, while leaving different requirements on the representations ultimately used for control.

\indent{\textbf{\textit{World Models and Latent-Action Conditioning.}}}
World models predict environment dynamics for planning and control~\citep{ha2018worldmodels,hafner2023dreamerv3}, with UniSim~\citep{yang2024unisim} and Cosmos~\citep{nvidia2025cosmos} scaling generative modeling to diverse video data. Action-conditioned architectures~\citep{acwmphys2026,wu2024ivideogpt} and robot datasets spanning diverse tasks and scenes~\citep{oxe2023,khazatsky2024droid} support learning from executable controls. To exploit action-unlabeled video, IGOR~\citep{chen2024igor} uses image-goal representations for both policy learning and video generation, while AdaWorld~\citep{gao2025adaworld} and DreamDojo~\citep{dreamdojo2026} use continuous latent actions for world-model pretraining and subsequent adaptation. CoLA-World~\citep{colaworld2025} couples quantized latent-action learning with a pretrained world model and analyzes distribution mismatch and codebook degeneration during real-action adaptation. CLAW~\citep{ayalew2026claw} jointly learns continuous actions and a diffusion world model, adversarially suppressing future-observation leakage. These approaches improve latent--world-model learning, but suppressing future appearance does not by itself exclude exogenous motion, and codebook stability does not determine which physical factors the codes represent.

\indent{\textbf{\textit{Action-Relevant and Structured Latent Representations.}}}
\citet{zhang2025whatdolams} analyze how reconstruction-driven learning can encode exogenous variation and observation-dependent shortcuts. LAOM~\citep{nikulin2025latentdistractors} studies distractors and shows that action decodability and usefulness as a policy target are distinct considerations. More recent methods impose explicit structure. ConLA~\citep{conla2026} combines category-based contrastive learning and temporal-reversal constraints in a quantized RGB-reconstruction LAM, while MVP-LAM~\citep{mvplam2026} uses cross-view reconstruction of frozen DINO features. Category agreement and cross-view consistency constrain semantic organization and viewpoint dependence, but do not by themselves separate all embodiment-controlled changes from other predictable variation. AC-LAM~\citep{aclam2026} imposes additive composition and evaluates identity, inverse consistency, and normalized zero-transition responses; these algebraic properties provide useful structure without uniquely determining the represented physical factors. MaskLAM~\citep{fechner2026masklam} restricts reconstruction to agent regions to reduce distractor encoding. DiLA~\citep{zhang2026dila} learns continuous actions through content--structure disentanglement and dynamics prediction in DINO feature space, supporting RGB generation and visual planning. Its separation of appearance from structural change leaves open how reliably transferred motion is assigned to the intended entity. These distinctions motivate evaluating latent actions according to their downstream use as embodied control conditions.

\indent{\textbf{\textit{Causal Perspectives on Bias Propagation.}}}
Invariant prediction~\citep{arjovsky2019irm}, shortcut learning~\citep{geirhos2020shortcut}, and causal confusion in imitation learning~\citep{dehaan2019causalconfusion} motivate examining which information a predictor uses and how that dependence affects its behavior. We investigate a specific mechanism in LAM-based ACWMs. CoCo~\citep{shi2026coco} addresses statistical shortcuts through counterfactual consistency constraints on action-conditioned world models. Source-specific visual information can be useful through the observation pathway yet also enter the latent action. If the world model relies on this information through its action condition, alignment with robot commands must accommodate variation that those commands cannot generally determine. CD-LAM targets this bias at its source through embodiment-centric reconstruction, action-centric contrastive learning, and latent-space calibration. We connect encoder diagnostics with action interventions and conditioned rollouts before and after \ratstage{}, evaluating how upstream representation correction affects controllability and whether its benefits persist under executable robot controls. Our study focuses on correcting the upstream latent-action representation and evaluating its effects before and after robot-action adaptation.

\indent{\textbf{\textit{Evaluating Controllability and Embodied Motion.}}}
Visual-fidelity metrics (\eg{} PSNR and FVD~\citep{unterthiner2018fvd}) do not by themselves establish whether a rollout follows its supplied action condition. Genie measures action sensitivity using $\Delta$PSNR~\citep{bruce2024genie}. MotionCtrl evaluates object-motion control with ObjMC~\citep{motionctrl2024}, while MotionPro measures trajectory alignment using mean-distance metrics, including MD-Vid computed with CoTracker~\citep{motionpro2025,cotracker2024}. Our \fdce{} metric compares foreground displacements between generated and reference rollouts, using SAM3 masks~\citep{carion2025sam3} and tracks from CoWTracker~\citep{lai2026cowtrackertrackingwarpinginstead}. We interpret this motion measure jointly with visual fidelity, latent diagnostics, and zero-action and target-action interventions to assess the downstream effects of latent-action debiasing.

==> 03_interface.tex <==
\section{Confounder Analysis on Latent Actions}
\label{sec:confounder}
In a LAM-based ACWM, \(z_t\) is the only action signal the world model receives during ACWM training, so any bias in \(z_t\) becomes a bias of the action condition itself. We first analyze why the reconstruction objective admits such bias, then verify the resulting failures in existing ACWMs.

\subsection{Why \texorpdfstring{a }{a }Reconstruction-centric Loss Admits Confounders}
For embodied ACWMs, \(z_t\) should act as the control signal whose dominant variation reflects key embodiment dynamics: body and object motion, contact, and displacement. A reconstruction-trained LAM does not enforce this property. Its objective only requires predictive sufficiency, \ie{} that \(z_t\) helps model \(p(o_{t+1}\mid o_t,z_t)\), so any transition-predictive factor can enter the latent:
\begin{equation}
    z_t = \mu_\phi(o_t,o_{t+1})
    \approx f(A_t, C_t, V_t),
    \label{eq:confounded-action-latent}
\end{equation}
where \(A_t\) denotes embodied action effects, \(C_t\) denotes scene context, and \(V_t\) denotes source-side visual factors such as background continuation and appearance continuity. The notation \(f(\cdot)\) records that nothing in the objective prevents \(z_t\) from carrying non-trivial dependence on \(C_t\) and \(V_t\) in addition to \(A_t\).
This induces \textbf{\textit{action-irrelevant confounding}}, illustrated in Figure~\ref{fig:causal}(d). Scene context and source-side visual factors are valid evidence in the observation history, where they help render the current scene. Once encoded into \(z_t\), however, they enter the action side of the model, and the condition partly specifies video continuation rather than embodiment dynamics. Robot action adaptation then inherits this contaminated latent space. A robot action \(u_t\) can ground the embodied dynamics in \(A_t\), but it cannot specify source-specific context, background continuation, or camera-like variation, so executable robot actions are forced into alignment with a partly non-actionable latent. This mismatch can increase the difficulty of robot-action alignment.

\subsection{Empirical Study on a Representative LAM-based ACWM}
\label{sec:interface-definitions}
\label{sec:observation}

We next check whether the analyzed failure appears in practice, using DreamDojo~\citep{dreamdojo2026} as a representative LAM-based ACWM. The evidence has two layers:

\noindent\textbf{{Weak Robot Action Following.}} After \ratstage{}, the generated embodiment dynamics should follow the conditioning action. However, DreamDojo ACWMs tend to violate this requirement in two basic settings, both of which keep the initial frame fixed and replace only the conditioning action. 
First, in the zero-action setting, we replace the conditioning action with zero, denoted \(\mathrm{do}(u_t=0)\). Although the embodiment motion should be suppressed, the rollout keeps moving (Figure~\ref{fig:zeroframe}). Second, under target-action transfer, where the conditioning action is replaced with one taken from a different target video, the rollout should reproduce the target embodiment dynamics, yet it does not (Figure~\ref{fig:transferaction}).
These examples indicate that the ACWM does not reliably follow the supplied robot actions. Both settings are interventions in the causal sense: the observation history is held fixed and only the action condition is replaced. These probes test the model's response to replacing the action condition while keeping the observation fixed, turning the disentanglement that Equation~(\ref{eq:confounded-action-latent}) calls for into a behavioral test, and Section~\ref{sec:exp-posttrain} applies the same two interventions.

\noindent\textbf{{Action-irrelevant Confounding in Latent Actions.}} We further examine the latent action space directly. A clean latent action space should satisfy three basic properties: (1) the zero-transition latent $z_t^{0}=\mu_\phi(o_t,o_t)$, encoded from a duplicated-frame pair, should remain close to zero; (2) camera-like image shifts should induce only small latent responses; and (3) local neighborhoods should reflect action similarity rather than shared visual context.  To quantify these three properties, we design corresponding evaluation metrics  (Appendix~\ref{app:metrics}) and apply them to the DreamDojo LAM encoder. As shown in Table~\ref{tab:latent-audit}, the DreamDojo LAM falls short of these desired properties and exhibits substantial bias: duplicated-frame pairs and synthetic camera shifts produce large latent responses, while same-episode visual context pulls latents closer even when their action primitives differ. The DreamDojo latent actions are thus significantly biased by action-irrelevant confounders.

\begin{figure}[!t]
\captionsetup{font=footnotesize}
\noindent\begin{minipage}[t]{0.49\linewidth}
\vspace{0pt}
\begin{subfigure}{\linewidth}
\centering
\includegraphics[width=\linewidth]{figures/zero.png}
\caption{Zero-action input.}
\label{fig:zeroframe}
\end{subfigure}

\vspace{8pt}
\captionsetup{type=table,position=above,justification=raggedright,singlelinecheck=false,skip=3pt}
\caption{\textbf{LAM encoder confounding audit}. A clean LAM encoder barely responds to action irrelevant changes (more details at  Table~\ref{tab:latent-audit-full}).}
\label{tab:latent-audit}
{\fontsize{8}{10}\selectfont
\setlength{\tabcolsep}{2pt}
\renewcommand{\arraystretch}{1.05}
\begin{tabular*}{\linewidth}{@{}l@{\extracolsep{\fill}}cc@{}}
\toprule
Diagnostic & DreamDojo & \method{} \\
\midrule
\multicolumn{3}{@{}l}{\emph{Zero-transition} (static pair $(o_t,o_t)$)}\\
\quad Rel.\ norm, median$\downarrow$ & $0.527$ & $\mathbf{0.043}$ \\
\quad Abs.\ norm, median$\downarrow$ & $3.119$ & $\mathbf{0.226}$ \\
\addlinespace[1pt]
\multicolumn{3}{@{}l}{\emph{Camera shift} (rel.\ norm, mean/median)}\\
\quad Horizontal$\downarrow$ & $0.555/0.536$ & $\mathbf{0.156/0.096}$ \\
\quad Vertical$\downarrow$ & $0.545/0.529$ & $\mathbf{0.110/0.064}$ \\
\addlinespace[1pt]
\multicolumn{3}{@{}l}{\emph{Action-neighbor structure}}\\
\quad Shortcut leakage$\downarrow$ & $0.151$ & $\mathbf{0.014}$ \\
\bottomrule
\end{tabular*}\par}
\end{minipage}\hfill
\begin{minipage}[t]{0.475\linewidth}
\setcounter{subfigure}{1}
\vspace{0pt}
\begin{subfigure}{\linewidth}
\centering
\includegraphics[width=\linewidth]{figures/transfer_new.png}
\caption{Transferred target action.}
\label{fig:transferaction}
\end{subfigure}

\vspace{4pt}
\captionsetup{type=figure,position=below,justification=raggedright,singlelinecheck=false}
\addtocounter{figure}{-1}
\caption{\textbf{Action-following failures under zero-input and target-action probes.} The initial frame is fixed and only the action is replaced. (a)~Zero action: the rollout still moves. (b)~Actions transferred from a target video (middle, green): the rollout (bottom, red) misses the target dynamics.}
\label{fig:action-intervention-failures}
\end{minipage}
\end{figure}


==> 04_method.tex <==
\section{CD-LAM: Causal Debiasing of Latent Actions}
\label{sec:method}
Section~\ref{sec:confounder} shows that reconstruction-only LAM training can confound latent actions. We propose CD-LAM, a causally motivated debiasing approach with an efficient staged fine-tuning pipeline.
\begin{figure}[!hbtp]
\centering
\includegraphics[width=1\linewidth]{figures/main_fig_iclr.pdf}
\caption{\textbf{Overview of CD-LAM.}
CD-LAM debiases the LAM's latent action space in three stages while keeping the downstream action conditioning format unchanged. \textbf{Stage 1 (LAM debiased fine-tuning)} debiases the LAM with the three CD-LAM objectives. \textbf{Stage 2 (\latstage{})} trains the ACWM on the debiased latent actions. \textbf{Stage 3 (\ratstage{})} aligns executable robot actions to the same space through a lightweight bridge.}
\label{fig:arch}
\end{figure}

\subsection{Design Principles}\label{sec:method-principles}
The analysis in Section~\ref{sec:confounder} leads to three design principles for keeping action-irrelevant factors out of the latent action space while visual context stays available through the observation path.

$\bullet$ \textbf{Embodiment-centric Reconstruction.} The reconstruction signal should emphasize regions tied to embodiment dynamics over background regions. \\
$\bullet$ \textbf{Action-centric Structure.} The latent action space should group videos with similar actions, not visually similar videos with different actions. \\
$\bullet$ \textbf{Calibrated Latent Space.} Duplicated-frame inputs should map to a designated zero-transition reference, while ordinary transitions retain enough variation to encode embodiment dynamics. 

CD-LAM implements these principles with three matching LAM objectives: embodiment-centric reconstruction (\(\mathcal L_{\mathrm{emb}}\)), action-centric contrastive learning (\(\mathcal L_{\mathrm{ctr}}\)), and latent space calibration (\(\mathcal L_{\mathrm{cal}}\)).

\subsection{CD-LAM Objective}

Given a transition \((o_t,o_{t+1})\), CD-LAM produces a debiased latent action
\begin{equation}
z_t^{\mathrm{CD}}=\mu_\phi(o_t,o_{t+1})\in\mathbb{R}^{d},
\label{eq:zcd}
\end{equation}
which is fed into the same ACWM conditioning format as the original DreamDojo latent.
The LAM is fine-tuned with
\begin{equation}
    \mathcal L_{\mathrm{CD}}
    =
    \mathcal L_{\mathrm{emb}}
    + \lambda_{\mathrm{ctr}}(k)\mathcal L_{\mathrm{ctr}}
    + \mathcal L_{\mathrm{cal}} .
    \label{eq:cdlam-total}
\end{equation}
 Here \(\lambda_{\mathrm{ctr}}(k)\) weights the contrastive term and varies with the training step \(k\) (we reserve \(t\) for frame time); the calibration term carries its own weights (Equation~(\ref{eq:action-norm-compact})).

\subsubsection{Embodiment-centric Reconstruction Loss}

We use an embodiment-centric weighted MSE for frame-pair reconstruction. Given a transition \((o_t,o_{t+1})\), CD-LAM predicts \(\hat{o}_{t+1}=D_\psi(o_t,z_t^{\mathrm{CD}})\) as in Equation~(\ref{eq:lam-autoencoder}).
Let \(M_t\in[0,1]^{h\times w}\) be the embodiment--object foreground mask
obtained by SAM3~\citep{carion2025sam3}, where \(h\times w\) is the frame resolution. We optimize the weighted reconstruction loss
{\small
\begin{equation}
    \mathcal L_{\mathrm{emb}}
    = \frac{1}{|\Omega|}\sum_{p\in\Omega}
    W_t(p)\,\big\|\hat{o}_{t+1}(p)-o_{t+1}(p)\big\|_2^2,
    \qquad
    W_t = \alpha_{\mathrm{fg}} M_t
        + \alpha_{\mathrm{bg}}(1-M_t).
    \label{eq:emb-rec}
\end{equation}}
where \(\Omega\) is the pixel grid and \(\alpha_{\mathrm{fg}}>\alpha_{\mathrm{bg}}\): embodiment and object errors cost more than background errors, while the nonzero background weight keeps global visual consistency.

\subsubsection{Action-centric Contrastive Learning}
Reconstruction alone treats each transition independently. CD-LAM adds a pairwise contrastive loss over coarse manipulation primitives so that action-consistent transitions remain close across visual contexts. Let \(v_i=\mathrm{norm}(r_\omega(z_i^{\mathrm{CD}}))\) with an auxiliary head \(r_\omega\), let \(s_{ij}=\tau\,v_i^\top v_j+b\) be their scaled cosine similarity, and let \(\mathcal P_\pm\) be the valid same-/different-primitive pairs in a batch:
{\small
\begin{equation}
\mathcal L_{\mathrm{ctr}}
=
\underbrace{\frac{1}{W_+}\sum_{(i,j)\in\mathcal P_+} w_{ij}\,\mathrm{softplus}(-s_{ij})}_{\text{pull same primitive together}}
+
\underbrace{\frac{1}{W_-}\sum_{(i,j)\in\mathcal P_-} w_{ij}\,\mathrm{softplus}(s_{ij})}_{\text{push different primitives apart}} .
\label{eq:contrast-compact}
\end{equation}
}


Each term is normalized by its own total pair weight, \(W_\pm=\max\!\big(1,\sum_{(i,j)\in\mathcal P_\pm}w_{ij}\big)\), and batches without positives contribute zero. The learned scale \(\tau\), bias \(b\)~\citep{zhai2023siglip}, and pair weights \(w_{ij}\) are specified in the released configuration.
The primitive labels are coarse verb-level categories (\eg{} pick--place, pour, open, close) obtained by mapping the datasets' task and verb annotations into a coarse primitive space (Appendix~\ref{app:verbs}) without involving any executable robot actions. Transitions without annotations still contribute to the reconstruction and calibration objectives.

\subsubsection{Latent Space Calibration}
The latent space calibration loss combines capacity control with zero-transition calibration:

\begin{equation}
    \mathcal L_{\mathrm{cal}}
    =
    \beta_{\mathrm{kl}}(k)\,\mathcal L_{\mathrm{KL\text{-}fb}}
    +
    \lambda_{\mathrm{zero}}\,\mathcal L_{\mathrm{zero}} ,~\quad
    \mathcal L_{\mathrm{zero}}
    =
    \mathbb E_{o_t}\big[\,[\rho_t-m_{\mathrm{zero}}]_{+}^{2}\,\big] .
    \label{eq:action-norm-compact}
\end{equation}

\noindent
The free-bit KL term \(\mathcal L_{\mathrm{KL\text{-}fb}}\) is a KL penalty applied only above a per-dimension free-bits floor. It provides capacity control while preserving variation among ordinary transitions. The zero-transition term \(\mathcal L_{\mathrm{zero}}\) acts on the relative norm \mbox{\(\rho_t=\|z_t^{0}\|_2/(\mathrm{sg}(s_\Delta)+\epsilon)\)} of the zero-transition latent \(z_t^{0}=\mu_\phi(o_t,o_t)\) (Section~\ref{sec:observation}), where \(s_\Delta\) is the running RMS norm of ordinary transition latents. It is nonzero only when \(\rho_t\) exceeds a small margin \(m_{\mathrm{zero}}\), so duplicated-frame inputs are encouraged toward the designated zero-transition reference. Here \(\mathrm{sg}(\cdot)\) is stop-gradient, \([x]_+=\max(x,0)\), and \(\beta_{\mathrm{kl}}(k)\), \(\lambda_{\mathrm{zero}}\) are term weights (Table~\ref{tab:loss}).

\subsection{Multi-stage Training}\label{sec:method-bridge}

CD-LAM is used in a three-stage training pipeline (Figure~\ref{fig:arch}):
% The first two stages operate on action-unlabeled video (LAM and \latstage), while the final stage introduces paired robot actions (\ratstage).

$\bullet$ \textbf{Stage 1 (LAM Debiased Fine-tuning).} We first fine-tune the LAM on videos without executable action labels using the CD-LAM objective of Equation~(\ref{eq:cdlam-total}) with only coarse task annotation. 

$\bullet$ \textbf{Stage 2 (ACWM Debiased Fine-tuning).} We then extract debiased latents \(z_t^{\mathrm{CD}}\) from videos and continue ACWM training under the conditioning of Equation~(\ref{eq:latent-acwm}), with \(z_t^{\mathrm{CD}}\) in place of \(z_t\). This adapts the world model to the debiased latent action space before executable robot actions are introduced.

$\bullet$ \textbf{Stage 3 (\Ratstage).}
Finally, for action labeled robot data \((o_t,u_t,o_{t+1})\), we align actions to the debiased latent action space. A lightweight MLP bridge \(g_\eta\) is trained to regress the gradient-stopped CD-LAM latent, \(g_\eta(u_t)\approx\mathrm{sg}\big(\mu_\phi(o_t,o_{t+1})\big)\). An auxiliary action readout with a cycle-consistency objective encourages the mapped latent to retain information about \(u_t\). During \ratstage{}, the ACWM receives \(\hat z_t=g_\eta(u_t)\), so robot actions enter the same debiased latent action space used in Stage 2. 


==> 05_experiments.tex <==
\section{Experiments}
\label{sec:experiments}\label{sec:exp}\label{sec:scale}

\subsection{Experimental Setup}
\label{sec:exp-axes}
\textbf{Models and baseline.}
We apply CD-LAM to DreamDojo~\citep{dreamdojo2026} at the 2B and 14B scales, which share a single latent action model, while keeping the downstream ACWM architecture, latent dimensionality, and conditioning interface unchanged. DreamDojo serves as the matched baseline to isolate the effect of latent-action debiasing within the same LAM--ACWM pipeline. For Stage 2, we continue the original DreamDojo training on the same video subset with matched update counts. For Stage 3, we compare against its released robot-action-adapted checkpoints under the same evaluation protocol. Recent latent-action methods span different levels of the learning stack, from alternative latent formulations and joint latent/world-model learning to policy/VLA pretraining~\citep{colaworld2025,ayalew2026claw,zhang2026dila}, so their reported scores also reflect differences in downstream architecture, action grounding, embodiment, and evaluation. We therefore use DreamDojo for the debiasing study, while LTX-2.3 and X-VLA serve as complementary transfer studies evaluating whether the action-conditioning interface and the learned latent representation remain useful beyond DreamDojo pipeline~\citep{hacohen2026ltx2,zheng2025xvla}.


\textbf{Training and data.} The main study runs on 128 H100 GPUs. Our three-stage fine-tuning starts from released DreamDojo checkpoints. By default, LAM debiasing uses 100h of DreamDojo pretraining human video, and robot-action adaptation uses approximately 300h of paired AgiBot video and actions~\citep{agibotworldcontributors2025agibotworldcolosseolargescale}. We evaluate latent-action rollouts on EgoDex~\citep{hoque2026egodexlearningdexterousmanipulation} and robot-action rollouts on held-out AgiBot clips. Training and evaluation details are provided in Appendix~\ref{app:setup}, with separate LTX and X-VLA protocols in Appendices~\ref{app:ltx} and~\ref{app:vla}.





\textbf{Metrics.} We evaluate visual fidelity with PSNR, SSIM~\citep{wang2004ssim}, and LPIPS~\citep{zhang2018perceptual}, and action following with Foreground Displacement Chamfer Error (\fdce{}). Pixel metrics alone do not certify action following: as Figure~\ref{fig:psnr-fdce} shows, high PSNR can coexist with incorrect embodiment motion. Following trajectory-based motion evaluation for controllable video generation~\citep{motionctrl2024,motionpro2025}, \fdce{} measures the symmetric Chamfer distance between generated and reference foreground displacement tracks in pixels; Figure~\ref{fig:metric-explainer} illustrates the computation and Appendix~\ref{app:metrics} provides the full definition. As a tracking-based proxy for action following, we interpret \fdce{} jointly with zero-action and target-action interventions, visual-fidelity metrics, and qualitative rollouts. For VLA policies, we report success rate.

\begin{figure}[!htbp]
\captionsetup{font=footnotesize,skip=5pt,justification=raggedright,singlelinecheck=false}
\noindent\begin{minipage}[t]{.49\linewidth}\vspace{0pt}
\captionsetup{justification=raggedright,singlelinecheck=false}
\centering

\includegraphics[width=0.70\linewidth]{figures/fdce_explainer.png}
\caption{\textbf{\fdce{} computation:} symmetric Chamfer distance of foreground displacement tracks.}
\label{fig:metric-explainer}
\end{minipage}\hfill\begin{minipage}[t]{.48\linewidth}\vspace{0pt}
\centering
\includegraphics[width=0.74\linewidth]{figures/scatter.pdf}
\caption{\textbf{Pixel-level fidelity does not certify action following.} PSNR explains only limited variance in FDCE (\(r=-0.38\), \(R^2=0.14\)). Each point is one rollout.}
\label{fig:psnr-fdce}
\end{minipage}
\end{figure}
\subsection{Latent Action Diagnostics (Stage 1)}
\label{sec:exp-lam}\label{sec:audit}%
We first audit the latent action before any world model rollout. This directly probes the upstream source identified in Section~\ref{sec:confounder}: whether the encoder responds to action-irrelevant confounders as if they were embodied action. Table~\ref{tab:latent-audit} shows that \method{} strongly reduces responses to action-irrelevant confounders: the median zero-transition response drops from 0.527 to 0.043, synthetic camera shifts induce 3.6--8.3\(\times\) smaller responses. Shortcut leakage is computed as the difference between the mean cosine similarity of same-episode pairs with different primitives and that of different-episode pairs with the same primitive. It drops from 0.151 to 0.014, indicating substantially less context-driven structure in the latent space.

\input{sections/_tab_wm_egodex.tex}

\subsection{\Latstage{} Rollouts (Stage 2)}
\label{sec:exp-pretrain}
We then evaluate ACWM rollouts conditioned on debiased LAM latents before introducing the robot-action bridge. Table~\ref{tab:wm-egodex} shows gains at two scales. Compared with the matched continued-training baseline, CD-LAM reduces FDCE by 42\% at 2B (34.00 to 19.63) and by 26\% at 14B (40.29 to 29.87) while also improving PSNR, SSIM, and LPIPS. Under target-action transfer \(\mathrm{do}(z_t=z_t^{\mathrm{tar}})\), FDCE drops by 21\% and 34\%, respectively, while pixel metrics show smaller, mixed changes. These results show that CD-LAM improves action following before robot-action alignment. We also found that scaling the baseline from 2B to 14B does not improve action following, whereas CD-LAM reduces FDCE at both scales.

\input{sections/_tab_posttrain_main.tex}




\subsection{\Ratstage{} Rollouts (Stage 3)}
\label{sec:exp-posttrain}\label{sec:main}\label{sec:repair}\label{sec:exp-wm}\label{sec:reuse}\label{sec:exp-interventions}\label{sec:interv}

Table~\ref{tab:posttrain-main} shows that CD-LAM also improves action following after robot-action adaptation. Under robot actions, CD-LAM reduces mean FDCE by 35\% at 2B (12.63 to 8.24) and 30\% at 14B (11.11 to 7.73), while improving median FDCE and all three visual-fidelity metrics. At 14B, CD-LAM achieves the best result in every column of the table, whereas baseline scaling is mixed: FDCE$_{\mathrm{med}}$ \emph{worsens} from 8.15 to 8.98 even as PSNR improves. Figure~\ref{fig:posttrain-panels} further shows that the gains span action categories and shift the rollout distribution toward lower FDCE and higher PSNR. Figure~\ref{fig:appendix-target-and-action} provides the full per-action breakdown and an additional target-action transfer example, while Figure~\ref{fig:cross_recon} shows representative rollouts at both scales. Under zero-input conditioning \(\mathrm{do}(u_t=0)\), residual FDCE decreases from 10.71 to 5.03 at 2B and from 9.36 to 2.18 at 14B. Zero FDCE corresponds to the static reference used in this probe. Under target-action transfer \(\mathrm{do}(u_t=u_t^{\mathrm{tar}})\), FDCE improves from 24.36 to 22.55 and from 24.82 to 21.11. Together, these interventions show that CD-LAM improves action following under both recorded and transferred actions while suppressing residual motion under zero-action conditioning.

\begin{figure}[!htbp]
\centering

\includegraphics[width=0.9\linewidth]{figures/post_panel.pdf}
\caption{\textbf{Action-following behavior after \ratstage{}, beyond aggregate scores.} (a) CD-LAM reduces FDCE in most action categories (full breakdown in Figure~\ref{fig:appendix-target-and-action}) at both 2B and 14B scales, so the gain is not concentrated in a single primitive. (b) On the 2B ACWM after \ratstage, CD-LAM shifts the rollout distribution toward lower FDCE and higher PSNR.}
\label{fig:posttrain-panels}
\end{figure}

\begin{figure}[!htb]
\noindent\begin{minipage}[c]{0.56\linewidth}
\centering
\includegraphics[width=\linewidth]{figures/com.pdf}
\end{minipage}\hfill
\begin{minipage}[c]{0.41\linewidth}
\captionsetup{font=footnotesize,justification=raggedright,singlelinecheck=false}
\caption{\textbf{Representative rollouts after \ratstage{} at 2B and 14B scale.} Rows: source video, DreamDojo, and CD-LAM at 2B and 14B; all model rows start from the same initial frame and receive the same robot action sequence.  DreamDojo's arm pose drifts from the ground-truth trajectory, and scaling to 14B does not repair the drift, whereas CD-LAM tracks the commanded motion at both scales. Scene appearance stays comparable, so the separation is in action following rather than visual quality. Colored overlays are row markers distinguishing the models, not model outputs.}
\label{fig:cross_recon}\label{fig:crossrecon}
\end{minipage}
\end{figure}

\subsection{\Ratstage{} Efficiency and Debiasing Data Scaling}

\label{sec:exp-scale}\label{sec:scale-results}\label{sec:disagree}\label{sec:lessmore}









Figure~\ref{fig:steps} shows that at 14B, CD-LAM reaches the DreamDojo reference within roughly 3k updates on FDCE and 4k updates on PSNR (more than 12\(\times\) fewer than the reference's 50k updates), and clearly surpasses it on both metrics by the 6k checkpoint in Table~\ref{tab:posttrain-main}. These results suggest that correcting the latent action representation before robot-action adaptation reduces the number of adaptation updates needed to reach the reference performance. Table~\ref{tab:scaling} evaluates the data side of the same effect. All tiers share the same 1k-step Stage-1 budget, so the comparison isolates data quantity at fixed compute. Even the 1h CD-LAM tier reduces FDCE$_{\mathrm{mean}}$ from 12.63 to 8.91, and the 1000h tier further lowers it to 7.97. The 1h tier captures about 80\% of the 1000h tier's FDCE improvement: limited debiasing data yields most of the gain, while more data refines action consistency.



\begin{figure}[H]
\captionsetup{font=footnotesize,skip=5pt,justification=raggedright,singlelinecheck=false}
\noindent\begin{minipage}[t]{.49\linewidth}\vspace{0pt}
\centering
\centering
\includegraphics[width=\linewidth]{figures/14b_paper_psnr_fdce_vs_dreamdojo_v4.pdf}
\captionsetup{justification=raggedright,singlelinecheck=false}
\captionsetup{position=below,skip=6pt}
\caption{\textbf{Robot adaptation efficiency.} 14B PSNR and FDCE over training steps. Dashed lines mark DreamDojo at 50k updates.}
\label{fig:steps}
\end{minipage}\hfill\begin{minipage}[t]{.48\linewidth}\vspace{0pt}
\centering
\captionof{table}{\textbf{Debiasing-data scaling at 2B.} All tiers use 1k Stage-1 updates and differ only in video hours. DreamDojo is the 50k-update robot adaptation reference.}
\label{tab:scaling}
\fontsize{8}{10}\selectfont
\setlength{\tabcolsep}{2pt}
\begin{tabular*}{\linewidth}{@{}l@{\extracolsep{\fill}}ccc@{}}
\toprule
Model & PSNR\,$\uparrow$ & FDCE$_{\text{mean}}$\,$\downarrow$ & FDCE$_{\text{med}}$\,$\downarrow$ \\
\midrule
DreamDojo       & $19.85$ & $12.63$ & $8.15$ \\
\method{}-1h    & $20.54$ & $8.91$  & $6.88$ \\
\method{}-10h   & $20.61$ & $8.87$  & $6.23$ \\
\method{}-100h  & $20.60$ & $8.24$  & $6.75$ \\
\method{}-1000h & $\mathbf{20.64}$ & $\mathbf{7.97}$ & $\mathbf{6.12}$ \\
\bottomrule
\end{tabular*}
\end{minipage}
\end{figure}

\subsection{Objective Ablation}
\label{sec:objective-ablation-results}\label{sec:ablation}
\begin{table}[!htbp]
\centering
\captionsetup{font=small,position=above,justification=raggedright,singlelinecheck=false,skip=6pt}
\caption{\textbf{CD-LAM objective ablation.} Each row omits the indicated LAM loss term. FG denotes FG-PSNR and $Cam.x/y$ are camera-shift responses.}
\label{tab:objective-ablation}
{\footnotesize
\setlength{\tabcolsep}{6pt}
\renewcommand{\arraystretch}{1.08}
\begin{tabular}{@{}lccccc@{}}
\toprule
Model & PSNR $\uparrow$ & FG $\uparrow$ & $Cam.x\downarrow$ & $Cam.y\downarrow$ & FDCE $\downarrow$ \\
\midrule
Full & \textbf{29.64} & \textbf{26.57} & \textbf{.133} & .101 & 17.23 \\
w/o $\mathcal L_{\mathrm{emb}}$ & 29.53 & 26.26 & .134 & \textbf{.100} & 18.40 \\
w/o $\mathcal L_{\mathrm{ctr}}$ & 29.64 & 26.57 & .134 & .101 & 19.07 \\
w/o $\mathcal L_{\mathrm{cal}}$ & 29.31 & 26.48 & .637 & .637 & \textbf{16.10} \\
\bottomrule
\end{tabular}\par}
\end{table}

Table~\ref{tab:objective-ablation} reports a separate ablation setup: PSNR and FG-PSNR evaluate Stage-2 rollouts, camera-shift norms probe the LAM, and FDCE evaluates Stage-3 rollouts. The $L_{\mathrm{emb}}$ ablation lowers FG-PSNR by 0.31 dB and increases FDCE by 1.17 px. Removing $L_{\mathrm{ctr}}$ leaves the reconstruction and camera-shift scores nearly unchanged but increases FDCE by 1.84 px. Removing the combined latent-space calibration term $L_{\mathrm{cal}}$ increases horizontal/vertical shifted-pair norms from 0.133/0.101 to 0.637/0.637 and lowers PSNR by 0.33 dB, while improving FDCE from 17.23 to 16.10. This reveals a trade-off: $L_{\mathrm{cal}}$ improves latent-space calibration and visual fidelity but does not uniformly improve downstream motion metrics, while the full model still achieves lower FDCE than the $L_{\mathrm{emb}}$ and $L_{\mathrm{ctr}}$ ablations. 






\subsection{Efficient Robot-Action Adaptation of a Pretrained Video Backbone}
\label{sec:ltx-enabling}
\begin{table*}[!hbpt]
\centering
\captionsetup{font=footnotesize,position=above,skip=3pt}
\caption{\textbf{Efficient adaptation on LTX-2.3.}
Training exposure and robot-action rollout performance relative to DreamDojo-14B.}
\label{tab:ltx-enabling}

{\fontsize{7.5}{8.5}\selectfont
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.05}

\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{lccc|ccc|ccc}
\toprule
& \multicolumn{3}{c|}{Latent-action pretraining}
& \multicolumn{3}{c|}{Robot-action adaptation}
& \multicolumn{3}{c}{Robot-action rollout} \\
\cmidrule(lr){2-4}
\cmidrule(lr){5-7}
\cmidrule(lr){8-10}

Model
& GPUs & Updates & \shortstack{Exposure\\Samples}
& GPUs & Updates & \shortstack{Exposure\\Samples}
& PSNR $\uparrow$
& FDCE$_{\mathrm{mean}}$ $\downarrow$
& FDCE$_{\mathrm{med}}$ $\downarrow$ \\
\midrule

DreamDojo 14B
& 256 H100 & 140k & 143.360M
& 128 H100 & 50k & 25.600M
& 20.01 & 11.11 & 8.98 \\

CD-LAM + LTX-2.3 22B
& 8  H200 & 60k & 3.840M
& 7  H200 & 28k & 1.568M
& \textbf{20.38} & 11.75 & \textbf{7.82} \\

\bottomrule
\end{tabular}
\end{adjustbox}
}
\end{table*}



We further test whether CD-LAM can efficiently adapt a generic pretrained video backbone into an embodied action-conditioned world model. Starting from LTX-2.3 22B, we perform only 60k latent-action pretraining updates, followed by 28k robot-action adaptation updates. This corresponds to 37.3 $\times$ fewer latent-action training sample exposures and 16.3 $\times$ fewer robot-action adaptation exposures than DreamDojo-14B. Despite this substantially reduced training exposure, the adapted LTX-2.3 achieves comparable robot-action rollout quality, with higher PSNR (20.38 vs.\ 20.01) and lower median FDCE (7.82 vs.\ 8.98). These results show that CD-LAM supports efficient adaptation of a pretrained video backbone to robot-action conditioning, achieving comparable rollout quality with substantially fewer training cost than DreamDojo-14B.


\subsection{Debiased Latent Actions as a Policy Pretraining Signal}
\label{sec:exp-vla}
\begin{figure}[!htbp]
\captionsetup{font=footnotesize,skip=5pt,justification=raggedright,singlelinecheck=false}
\noindent\begin{minipage}[t]{.51\linewidth}\vspace{0pt}
\centering
\includegraphics[width=\linewidth]{figures/vla/vla_learning_curves.pdf}
\caption{\textbf{Policy learning curves.} LIBERO (left) and LIBERO-Plus (right). Means, individual seeds, and min--max bands over three paired seeds; fixed subsets of 200 and 280 episodes. Full-benchmark comparisons use the 80k endpoints.}
\label{fig:vla-steps}
\end{minipage}\hfill\begin{minipage}[t]{.47\linewidth}\vspace{0pt}
\centering
\centering
\captionsetup{font=footnotesize,justification=raggedright,singlelinecheck=false,skip=6pt}
\captionof{table}{\textbf{X-VLA policy success (\%).} CD-LAM improves over DreamDojo LAM on LIBERO, LIBERO-Plus, and RoboTwin C2R.}
\label{tab:vla-main}
{\fontsize{7.5}{9.5}\selectfont
\setlength{\tabcolsep}{2pt}
\renewcommand{\arraystretch}{1.08}
\begin{tabular*}{\linewidth}{@{}l@{\extracolsep{\fill}}cc|cc@{}}
\toprule
\multirow{2}{*}{Training} & \multirow{2}{*}{LIBERO} & \multirow{2}{*}{\shortstack{LIBERO-\\Plus}} & \multicolumn{2}{c}{RoboTwin C2R} \\
& & & Clean & Random \\
\midrule
X-VLA & 98.05 & 69.74 & 85.67 & 25.00 \\
\arrayrulecolor{black!25}\midrule\arrayrulecolor{black}
DreamDojo LAM & 95.72 & 75.69 & 84.00 & 28.83 \\
CD-LAM & \textbf{96.30} & \textbf{78.25} & \textbf{86.67} & \textbf{33.83} \\
\midrule
$\Delta$ (pp) & +0.58 & +2.56 & +2.67 & +5.00 \\
\bottomrule
\end{tabular*}}
\end{minipage}
\end{figure}





Finally, we compare X-VLA policies trained with latent actions from either DreamDojo LAM or CD-LAM, using matched recipes within each benchmark (Table~\ref{tab:vla-main}). Across three paired post-training seeds, CD-LAM improves LIBERO success from 95.72\% to 96.30\% and LIBERO-Plus overall success from 75.69\% to 78.25\%, with positive mean gains across all seven perturbation categories. On RoboTwin~2.0, we evaluate C2R robustness on a predefined 12-task subset comprising ten eligible tasks with the largest public X-VLA clean-to-random gaps and two anchor tasks to assess policy robustness after latent-action pretraining. With  CD-LAM, randomized-scene success increases from 28.8\% to 33.8\%, with comparable clean performance (84.0\% vs.\ 86.7\%). These results show that CD-LAM also improves downstream policy success. Full protocols, task-selection criteria, and task-level results are provided in Appendix~\ref{app:vla}.
Figure~\ref{fig:vla-steps} shows the three paired post-training trajectories on fixed monitoring subsets; the full-benchmark comparisons above use the fixed 80k endpoints.


\FloatBarrier

==> 08_conclusion.tex <==
% \enlargethispage{2\baselineskip}
\section{Conclusion}\label{sec:conclusion}
We presented CD-LAM, a causally motivated framework that improves world model controllability by reducing visual bias in latent action representations. Across 2B and 14B backbones, CD-LAM improves action following, visual fidelity, and adaptation efficiency, with benefits persisting from latent action conditioning to executable robot controls. Experiments with LTX-2.3 and X-VLA further demonstrate its applicability to video model adaptation and policy learning. Together, these findings identify upstream representation bias as a practical obstacle to downstream control and show that correcting it yields benefits across models and tasks. By correcting bias in latent actions, CD-LAM offers a practical path toward more controllable world models and more robust embodied policies.

==> _tab_posttrain_main.tex <==
\begin{table}[!htb]
\centering\footnotesize
\setlength{\tabcolsep}{3.2pt}\renewcommand{\arraystretch}{1.2}
\caption{\textbf{Robot action rollouts and interventions on AgiBot (Stage 3).} Zero-action FDCE is residual motion w.r.t.\ the static initial frame. DreamDojo: released 50k-update checkpoints.}
\label{tab:posttrain-recon-2b14b}\label{tab:ego}\label{tab:posttrain-main}\label{tab:interventions}\label{tab:latent-interventions}

\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{@{}llccccccc@{}}
\toprule
& & \multicolumn{5}{c}{robot action \(u_t\) rollout} & \(\mathrm{do}(u_t=0)\) & \(\mathrm{do}(u_t=u_t^{\mathrm{tar}})\) \\
\cmidrule(lr){3-7}\cmidrule(lr){8-9}
Backbone & Model & FDCE$_{\text{mean}}$\,$\downarrow$ & FDCE$_{\text{med}}$\,$\downarrow$ & PSNR\,$\uparrow$ & SSIM\,$\uparrow$ & LPIPS\,$\downarrow$
 & FDCE\,$\downarrow$ & FDCE\,$\downarrow$ \\
\midrule
\multirow{2}{*}{2B}
& DreamDojo & $12.63$ & $8.15$ & $19.85$ & $0.798$ & $0.271$ & $10.71$ & $24.36$ \\
& \method{} & $\mathbf{8.24}$ & $\mathbf{6.75}$ & $\mathbf{20.60}$ & $\mathbf{0.806}$ & $\mathbf{0.269}$ & $\mathbf{5.03}$ & $\mathbf{22.55}$ \\
\midrule
\multirow{2}{*}{14B}
 & DreamDojo & $11.11$ & $8.98$ & $20.01$ & $0.808$ & $0.263$ & $9.36$ & $24.82$ \\
& \method{} & $\mathbf{7.73}$ & $\mathbf{5.99}$ & $\mathbf{21.01}$ & $\mathbf{0.818}$ & $\mathbf{0.247}$ & $\mathbf{2.18}$ & $\mathbf{21.11}$ \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table}


==> _tab_wm_egodex.tex <==
\begin{table}[!htbp]
\caption{\textbf{Latent action conditioned rollouts after \latstage.}
Left: conditioned on \(z_t\) from the video transition. Right: target-action transfer \(\mathrm{do}(z_t=z_t^{\mathrm{tar}})\).}
\label{tab:wmego}\label{tab:wm-egodex}

\centering\footnotesize
\setlength{\tabcolsep}{3.2pt}\renewcommand{\arraystretch}{1.1}
\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{@{}llcccccccc@{}}
\toprule
& & \multicolumn{4}{c}{latent action \(z_t\) rollout} & \multicolumn{4}{c}{ \(\mathrm{do}(z_t=z_t^{\mathrm{tar}})\) } \\
\cmidrule(lr){3-6}\cmidrule(lr){7-10}
Backbone & Model & \fdce{}\,$\downarrow$ & PSNR\,$\uparrow$ & SSIM\,$\uparrow$ & LPIPS\,$\downarrow$
      & PSNR\,$\uparrow$ & SSIM\,$\uparrow$ & LPIPS\,$\downarrow$ & \fdce{}\,$\downarrow$ \\
\midrule
\multirow{2}{*}{2B}
 & DreamDojo      & $34.00$ & $20.88$ & $0.780$ & $0.413$ & $13.02$ & $\mathbf{0.598}$ & $0.643$ & $42.74$ \\
 & \method{}  & $\mathbf{19.63}$ & $\mathbf{24.29}$ & $\mathbf{0.827}$ & $\mathbf{0.308}$ & $\mathbf{13.15}$ & $0.588$ & $\mathbf{0.600}$ & $\mathbf{33.81}$ \\
\midrule
\multirow{2}{*}{14B}
 & DreamDojo & $40.29$ & $21.04$ & $0.792$ & $0.398$ & $\mathbf{13.11}$ & $0.593$ & $0.631$ & $50.27$ \\
 & \method{}  & $\mathbf{29.87}$ & $\mathbf{23.18}$ & $\mathbf{0.814}$ & $\mathbf{0.342}$ & $13.03$ & $\mathbf{0.597}$ & $\mathbf{0.617}$ & $\mathbf{33.22}$ \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table}

